On the Efficiency of the Information Networks in Social Media

Social media sites are information marketplaces, where users produce and consume a wide variety of information and ideas. In these sites, users typically choose their information sources, which in turn determine what specific information they receive, how much information they receive and how quickly this information is shown to them. In this context, a natural question that arises is how efficient are social media users at selecting their information sources. In this work, we propose a computational framework to quantify users' efficiency at selecting information sources. Our framework is based on the assumption that the goal of users is to acquire a set of unique pieces of information. To quantify user's efficiency, we ask if the user could have acquired the same pieces of information from another set of sources more efficiently. We define three different notions of efficiency -- link, in-flow, and delay -- corresponding to the number of sources the user follows, the amount of (redundant) information she acquires and the delay with which she receives the information. Our definitions of efficiency are general and applicable to any social media system with an underlying information network, in which every user follows others to receive the information they produce. In our experiments, we measure the efficiency of Twitter users at acquiring different types of information. We find that Twitter users exhibit sub-optimal efficiency across the three notions of efficiency, although they tend to be more efficient at acquiring non-popular than popular pieces of information. We then show that this lack of efficiency is a consequence of the triadic closure mechanism by which users typically discover and follow other users in social media. Finally, we develop a heuristic algorithm that enables users to be significantly more efficient at acquiring the same unique pieces of information.

==> sec/sec_intro_recent.tex <==
During the last decades, the creation, distribution, acquisition and manipulation of information has become a significant economic, political and cultural activity~\cite{castells2011rise}.
%
In this context, people \rem{has}\rev{have} increasingly \rem{relied}\rev{depended} on the Web for finding information of \rem{public}\rev{their} interest as well as keeping up to date with \rem{last}\rev{latest} breaking news. \rem{In other words,}\rev{As such,} the Web has become people'{}s ``first reads," \ie, their default source of information~\cite{kohut2008internet}.
%
A broad spectrum of websites has emerged to serve that purpose, ranging from online news media outlets such as the New York Times or CNN, specialized blogs and online 
magazines such as Engadget or Gizmodo, to digital encyclopedias such as Wikipedia. 
%
Importantly, in most of these sites, information is often curated by editorial boards, professional journalists, or renowned experts with a recognized reputation.

The advent of social media {and social networking sites }is changing \rem{dramatically}\rev{profoundly} the way in which people acquire\- and consume information. 
%
Social \rem{media}\rev{networking} sites such as Twi\-tter, \rem{Pinterest}\rev{Google Scholar}, or Tumblr have become global platforms for \rem{public self-expression and conversation}\rev{information sharing}.\rem{; more formally,}
These sites can be viewed as large 
information networks where nodes (\ie, users) \rem{create}\rev{produce} and consume information~\cite{bosagh2013precision,kwak2010twitter},
%
playing therefore the role of information curators by deciding which information to \emph{post} \rev{and} which other nodes in the network to \emph{fo\-llow} \rev{\cite{christakis2010social}.}
%
This entails serious challen\-ges as well as raises many important questions, which have not been addressed until very recently.
%
For example, users tend to follow \rem{sets of users that provide redundant information, often too many, perhaps afraid of missing out}\rev{too many other users and receive redundant information~\cite{babaei15icwsm}, \rem{often too many, }perhaps afraid of missing out~\cite{hodas2012visibility}}. \rem{As a consequence}\rev{As a result}, they become overloaded and 
effectively miss the information they were interested in~\cite{gomez14icwsm,Lerman14plosone}.
%
Moreover, since information is not professionally curated, its high-quality, relevance and credibility are at stake\rem{ and need to be assessed to avoid the spread of misinformation and false rumors}~\cite{agichtein2008finding,castillo2011information,source15aistats}.
%
\rem{Finally}\rev{Moreover}, the large amounts of small short lived pieces of information present in social media require developing new techniques for news aggregation~\cite{lerman2007social}, summarization~\cite{o2010tweetmotif}, and recommendation~\cite{abel2011analyzing}.

% fundamental questions
\rem{The present work is motivated by two fundamental indispensable  questions that, perhaps surprisingly, are barely hardly understood:}\rev{The motivation behind this work originates from two fundamental 
questions.}
%
i) How \emph{efficient} are the users of a social media site at selecting which other users to follow to acquire information of their interest? And, ii) can we design an information lossless rewiring heuristic method to enable a user 
to be more efficient at acquiring the same pieces of information? 
%
The answers to these questions are intertwined, since we can think of the structure of the information networks in social media sites as the output of a network formation game~\cite{kearns2012experiments}, where 
nodes (\ie, users) link other nodes to solve a specific task (\ie, \rem{acquire relevant information}\rev{acquire information relevant to the user}).
%
In this work, we \rem{define}\rev{propose} a general computational framework to quantify and optimize users'{} efficiency at acquiring information.

% more specific
With such a framework in place, we analyze the efficiency in social media as information systems, answering several important additional questions:
% efficiency vs coverage
When a user follows one more person, she aims to cover more information, however, what is the typical relation between information co\-ve\-rage and efficiency? Is
covering popular information in the heavy tail of popularity distribution different to covering non-popular information in the head of the distribution?
% discoverability via triadic closure
Both triadic closure~\cite{simmel1950sociology,granovetter1973strength,RomKle10} and information diffusion~\cite{weng2013role,myers2014bursty,AntDov13} have been shown to be major forces that trigger new 
links in social networks, however, are these mechanisms leading users to follow non-optimal sets of information sources? If so, to which extent?
%
People trade-off efficiency for simplicity when discovering content in information systrems such as Wikipedia~\cite{west2012automatic,west2012human}, however, can we find a similar trade-off when selecting information 
sources in user-generated information networks such as Twitter?

%  set covers
In this \rem{paper}\rev{study}, we define an intuitive computational framework that \rem{allows}\rev{enables} us to quantify Twitter users'{} efficiency at acqui\-ring information.
%
Our framework is based on the following key concept: given a set of unique ideas, pieces of information, or more generally, \emph{memes} $\Ical$ spreading through an information network, there is an \textit{optimal} set of nodes that, if followed, would \rem{allow}\rev{enable} us to get to know $\Ical$.
%
\rem{However}\rev{Naturally}, this \rem{key }concept relies on defining what is an optimal set. Here, we consider three notions of optimality, which lead to three types of efficiencies:
%
\begin{itemize}
% \denselist
%
\item[I.] {\bf Link efficiency.} The optimal set $\Ucal^{l}(\Ical)$ is the one that contains the smallest number of users. Then, we compute link efficiency by comparing the number of people a user follows, i.e., 
the number of \emph{followees}, with the size of the optimal set $\Ucal^{l}(\Ical)$. Finding the optimal set reduces to a minimum set cover problem, which can be solved using a well-known and efficient greedy algorithm 
with provable guarantees~\cite{johnson1973approximation}.

\item[II.] {\bf In-flow efficiency.} The optimal set $\Ucal^{f}(\Ical)$ is the one that provides the least amount of tweets per time unit. Then, we compute in-flow efficiency by comparing the amount of tweets
per time unit a user receives from the people she follows with the amount of tweets per time unit she would have received by following the users in the optimal set $\Ucal^{f}(\Ical)$. Finding the optimal set reduces
to a minimum weighted set cover problem, which again can be solved efficiently with provable guarantees~\cite{johnson1973approximation}.

\item[III.] {\bf Delay efficiency.} The optimal set $\Ucal^{t}(\Ical)$ is the one that provides the memes as early as possible. Then, we compute delay efficiency by comparing the average delay per meme that the user achieves through
the people she follows with the average delay she would achieve by following the users in the optimal set. Here, we define the delay at acquiring a meme in a social media system as the difference between the time when 
the user received the meme in her timeline and the time when the meme was first mentioned by a user in the social media system.
\end{itemize}
Although the concept of link efficiency has been previously introduced in\rem{our poster paper}~\cite{babaei15icwsm}, here we extend \rem{this piece of work}\rev{it} to account for other definitions of efficiency, i.e., in-flow and delay efficiency. \rev{Other related works, to the best of our knowledge, do not compare optimal sets to the sets followed by real users~\cite{leskovec2007cost}. Here, using our definitions of efficiency,} we study the tradeoff between efficiency and discoverability of the optimal set of \emph{followees}.
Our analysis \rem{yields}\rev{provides} several insights that do not only \rem{reveal}\rev{disclose} how efficient are users in social media at acquiring information, but also help us in understanding the influence different factors have on the efficiency of social media users at acquiring information:

\begin{enumerate}
\item We find that users acquire information sub-optimally with respect to the above notions of efficiency.

\item There is a trade-off between information coverage and information efficiency. While the popular pieces of information can be acquired through few users within low volume of posts, less popular information requires 
following many different users within high volume of posts.

\item Users trade followees'{} discoverability for information effi\-cien\-cy. While, for a typical Twitter user, many people in her original ego-network may be discovered by triadic closure, very few people in the optimized efficient 
ego-networks can be discovered in that way.

\item We introduce an information lossless rewiring heuristic me\-thod that significantly improves both user'{}s inflow and delay efficiencies at acquiring the same unique pieces of information.
%
\end{enumerate}
%
Moreover, our empirical findings shed light on how our notion of efficiency relates to different aspects of pieces of information (\eg, popularity) and a user'{}s ego-network structure (\eg, triangle closure, clustering coefficient). 
%
However, an important re\-mai\-ning question, left as potential future work, is to \rem{investigate}\rev{explore} how users'{} effi\-cien\-cy relates to their level of activity and engagement within the online social media system~\cite{shaping14nips}.

